Exploring Jamming and Hijacking Attacks for Micro Aerial Drones

Recent advancements in drone technology have shown that commercial off-the-shelf Micro Aerial Drones are more effective than large-sized drones for performing flight missions in narrow environments, such as swarming, indoor navigation, and inspection of hazardous locations. Due to their deployments in many civilian and military applications, safe and reliable communication of these drones throughout the mission is critical. The Crazyflie ecosystem is one of the most popular Micro Aerial Drones and has the potential to be deployed worldwide. In this paper, we empirically investigate two interference attacks against the Crazy Real Time Protocol (CRTP) implemented within the Crazyflie drones. In particular, we explore the feasibility of experimenting two attack vectors that can disrupt an ongoing flight mission: the jamming attack, and the hijacking attack. Our experimental results demonstrate the effectiveness of such attacks in both autonomous and non-autonomous flight modes on a Crazyflie 2.1 drone. Finally, we suggest potential shielding strategies that guarantee a safe and secure flight mission. To the best of our knowledge, this is the first work investigating jamming and hijacking attacks against Micro Aerial Drones, both in autonomous and non-autonomous modes.

==> Table/Summary.tex <==
\begin{table*}[!h]
\centering
\caption{Summary of the wireless attacks against the Crazyflie drone in autonomous and non-autonomous modes. For each flight mode, we provide a description of the Crazyflie drone and the Ground Control Station status along with the user and adversary's capabilities.}
\label{Summary}
\resizebox{\textwidth}{!}{ 
\begin{tabular}{llllll}
\hline
\multicolumn{1}{|l|}{\textbf{Wireless Attack}} & \multicolumn{1}{c|}{\textbf{Flight Mode}} & \multicolumn{1}{c|}{\textbf{Crazyflie Drone Status}}                                                                                                     & \multicolumn{1}{l|}{\textbf{Ground Control Station Status}}                                                                         & \multicolumn{1}{l|}{\textbf{User Capabilities}}                                                             & \multicolumn{1}{l|}{\textbf{Adversary's Capabilities}}                                                                                      \\ \hline
\multicolumn{1}{|l|}{Eavesdropping}            & \multicolumn{1}{l|}{Auton.}           & \multicolumn{1}{l|}{Regular operation of the GCS.}                                                                                             & \multicolumn{1}{l|}{Regular operation of the GCS.}                                                                                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user has a full control \\ on the drone.\end{tabular}}   & \multicolumn{1}{l|}{The adversary gathers sensitive data.}                                                                                  \\ \hline
\multicolumn{1}{|l|}{Eavesdropping}            & \multicolumn{1}{l|}{Non-Auton.}       & \multicolumn{1}{l|}{Regular operation of the GCS.}                                                                                             & \multicolumn{1}{l|}{Regular operation of the GCS.}                                                                                  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user has a full control \\ on the drone.\end{tabular}}   & \multicolumn{1}{l|}{The adversary gathers sensitive data.}                                                                                  \\ \hline
\multicolumn{1}{|l|}{Jamming}                  & \multicolumn{1}{l|}{Auton.}           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The drone crashes down \\ (failure in the rotors).\end{tabular}}                                & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The connection between the GCS\\ and the drone cannot be established.\end{tabular}}  & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user cannot control \\ the drone.\end{tabular}}          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The adversary disrupts the flight \\ mission and causes damage to the drone.\end{tabular}}   \\ \hline
\multicolumn{1}{|l|}{Jamming}                  & \multicolumn{1}{l|}{Non-Auton.}       & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The drone freezes during the mid-flight \\ (the rotors are operational).\end{tabular}}          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The connection between the GCS and \\ the drone cannot be established.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user cannot control \\ the drone.\end{tabular}}          & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The adversary disrupts the flight \\ mission and freezes the drone in the air.\end{tabular}} \\ \hline
\multicolumn{1}{|l|}{Hijacking}                & \multicolumn{1}{l|}{Auton.}           & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The drone crashes down, then wait for \\ the connection link to be reestablished.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The connection between the GCS and \\ the drone cannot be established.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user cannot send \\ commands to the drone.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The adversary take full control of \\ the drone after it crashes down.\end{tabular}}         \\ \hline
\multicolumn{1}{|l|}{Hijacking}                & \multicolumn{1}{l|}{Non-Auton.}       & \multicolumn{1}{l|}{The drone remains operational.}                                                                                            & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The connection between the GCS and \\ the drone cannot be established.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The user cannot send \\ commands to the drone.\end{tabular}} & \multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}The adversary take full control of\\ the drone.\end{tabular}}                                \\ \hline
                                               &                                           &                                                                                                                                                &                                                                                                                                     &                                                                                                             &                                                                                                                                            
\end{tabular}
}
\end{table*}

